Not Your Average App: A Large-scale Privacy Analysis of Android Browsers

The transparency and privacy behavior of mobile browsers has remained widely unexplored by the research community. In fact, as opposed to regular Android apps, mobile browsers may present contradicting privacy behaviors. On the one end, they can have access to (and can expose) a unique combination of sensitive user data, from users' browsing history to permission-protected personally identifiable information (PII) such as unique identifiers and geolocation. However, on the other end, they also are in a unique position to protect users' privacy by limiting data sharing with other parties by implementing ad-blocking features. In this paper, we perform a comparative and empirical analysis on how hundreds of Android web browsers protect or expose user data during browsing sessions. To this end, we collect the largest dataset of Android browsers to date, from the Google Play Store and four Chinese app stores. Then, we developed a novel analysis pipeline that combines static and dynamic analysis methods to find a wide range of privacy-enhancing (e.g., ad-blocking) and privacy-harming behaviors (e.g., sending browsing histories to third parties, not validating TLS certificates, and exposing PII -- including non-resettable identifiers -- to third parties) across browsers. We find that various popular apps on both Google Play and Chinese stores have these privacy-harming behaviors, including apps that claim to be privacy-enhancing in their descriptions. Overall, our study not only provides new insights into important yet overlooked considerations for browsers' adoption and transparency, but also that automatic app analysis systems (e.g., sandboxes) need context-specific analysis to reveal such privacy behaviors.

==> ccs_xml.tex <==
% TODO: replace this section with code generated by the tool at https://dl.acm.org/ccs.cfm
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002978.10003029.10011703</concept_id>
<concept_desc>Security and privacy~Usability in security and privacy</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc{Security and privacy~Use https://dl.acm.org/ccs.cfm to generate actual concepts section for your paper}
% -- end of section to replace with generated code

\keywords{template; formatting; pickling} % TODO: replace with your keywords


==> key_findings.tex <==
\section{Summary of Findings}


% \ml{can we emphasize some of the finding? (or ``type'' of finding)}
% \ml{also I find the placement of the related work section weird. how about we split out some of the concluding discussion and merge it with the key findings in a proper discussion section? we then can keep the conclusions pretty short.}




% Intro finding summary
%
%\item We find that \easylistBrowsersPercentage{} of browsers enhance privacy by
%  blocking tracking scripts by default. Similarly, \percTrackerBlockers{}
%  of browsers block scripts that access protected JavaScript APIs.
%
%\item We see that most browsers do not default to HTTP\textbf{S} (only \domainHttpsBrowsersPercentage{}
%  of browsers do so) and that \httpsFailPercentage{} of browsers do not properly
%  validate TLS certificates, making them vulnerable to person-in-the-middle attacks.
%  
%\item We find that \oneLib{} of browsers contain at least one
%  third-party library related to advertisement and tracking,
%  and that these
%  libraries are often responsible for browsers requesting dangerous permissions.
%  Furthermore, our run-time behavior analysis shows that 135 browsers share
%  PII with other parties over the Internet, and that \totalHistoryLeakBrowsers{} browsers
%  do the same for browsing history. While \historyLeakersFeatures{}
%  of these browsers share this information for a specific feature (such as web search
%  APIs), we find that \historyLeakersWithPII{} send it alongside
%  personal data (thus harming user privacy).
%  
%\item We conduct a multidimensional analysis of individual browsers to understand 
%    their overall privacy disposition. We find that few browsers uniformly improve privacy 
%    (FOSS Browser), while many exhibit multiple harms. We also find mixed behaviors: of the 
%    277 browsers that block tracking content, we see that 195 also allow tracking requests, 
%    63 expose PII, 38 share browsing history, and 20 fail to validate certificates.


==> plots/behavioral_analysis_overview.tex <==
\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Summary of observed browser behaviors.}
    \resizebox{.9\columnwidth}{!}{%
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={test,apps,percentage},
        columns/test/.style={column name=\textbf{Behavior}, column type={l}},
        columns/apps/.style={column name=\textbf{\# of browsers}, column type={r}},
        columns/packs/.style={column name=\textbf{\# of packages}, column type={r}},
        columns/percentage/.style={column name=\textbf{\% of browsers}, column type={r}},
        every head row/.style={after row=\midrule},
        %every last row/.style={after row=\bottomrule},
      ]{plots/behavioral_analysis_overview.csv}}
    \label{table:behavioral_analysis_overview}
\end{table}


==> plots/browser_engines.tex <==
\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Browsers engines based on User-Agent strings.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={engine,apps,percentage},
        columns/engine/.style={column name=\textbf{Browser Engine}, column type={l}},
        columns/apps/.style={column name=\textbf{Number of Browsers}, column type={r}},
        columns/packs/.style={column name=\textbf{\# of Packages}, column type={r}},
        columns/percentage/.style={column name=\textbf{Percentage}, column type={r}},
        every head row/.style={after row=\midrule},
        %every last row/.style={before row=\midrule,after row=\bottomrule},
    ]{plots/browser_engines.csv}
    \label{table:browser_engines}
\end{table}


==> plots/cn_ru_list.tex <==
\begin{table}[h!]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \scriptsize
    \caption{Websites for censorship tests from Citizen Lab.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={category,china,russia},
        columns/russia/.style={column name=\textbf{Russia}, column type={r}},
        columns/china/.style={column name=\textbf{China}, column type={r}},
        columns/category/.style={column name=\textbf{Category}, column type={l}},
        every head row/.style={after row=\midrule},
        %every last row/.style={after row=\bottomrule},
    ]{plots/cn_ru_list.csv}
    \label{table:cn_ru_list}
\end{table}


==> plots/fsmon_pii.tex <==

\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Number of browsers across datasets writing PII (by type) to the external storage (\ie{} the SD card).}
    
    \resizebox{\linewidth}{!}{%
    \pgfplotstabletypeset[
        every head row/.style={ after row=\midrule },
        every last row/.style={ before row=\midrule },
        col sep=comma,
        string type,
        columns={pii,play_brow,pre_brow,alt_brow,all_brow},
        columns/pii/.style={column name=\textbf{PII Type}, column type={l}},
        columns/play_brow/.style={column name=\textbf{Google Play}, column type={r}},
        columns/play_pack/.style={column name=\textbf{P}, column type={r}},
        columns/pre_brow/.style={column name=\textbf{Pre-installed}, column type={r}},
        columns/pre_pack/.style={column name=\textbf{P}, column type={r}},
        columns/alt_brow/.style={column name=\textbf{Alt. Markets}, column type={r}},
        columns/alt_pack/.style={column name=\textbf{P}, column type={r}},
        columns/all_brow/.style={column name=\textbf{All Origins}, column type={r}},
        columns/all_pack/.style={column name=\textbf{P}, column type={r}}
    ]{plots/fsmon_pii.csv}}
    \label{table:fsmon_pii}
    
\end{table}


==> plots/history_end_host_full.tex <==
\begin{table}[t!]
    \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Number of unique browsers sharing browsing history and PII
      together, allowing other parties to link the history to a unique user
      (* First party).}
    %\resizebox{\linewidth}{!}{
    \pgfplotstabletypeset[
        every head row/.style={
            %before row={
            %    \toprule
            %},
            after row=\midrule
        },
        every last row/.style={
          before row={
            \midrule
            \rowcolor{white}
          },
          %after row=\bottomrule
        },
        col sep=colon,
        string type,
        columns={
            company,
            browsers,
            location_info,
            Ad_id
            %imei,
            %device_mac
        },
        columns/location_info/.style={
            column name=\textbf{Location},
            column type={r}
        },
        columns/device_mac/.style={
            column name=\textbf{MAC$\textsubscript{D}$},
            column type={r}
        },
        columns/Ad_id/.style={
            column name=\textbf{AdID},
            column type={r}
        },
        columns/imei/.style={
            column name=\textbf{IMEI},
            column type={r}
        },
        columns/wifi_mac/.style={
            column name=\textbf{MAC$\textsubscript{W}$},
            column type={r}
        },
        columns/screen_info/.style={
            column name=\textbf{Screen},
            column type={r}
        },
        columns/company/.style={
            column name=\textbf{Destination},
            column type={l}
        },
		columns/packages/.style={
            column name=\textbf{\# of P},
            column type={r}
        },
        columns/browsers/.style={
            column name=\textbf{\# of Browsers},
            column type={r}
        } 
    ]{plots/history_end_host_full.csv}
    %}
    \label{table:history_end_hosts_full}
\end{table}



==> plots/https_fail.tex <==
\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Packages failing the HTTPS test, along with the number of browser versions affected for each package.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={package,count},
        columns/package/.style={column name=\textbf{Package}, column type={l}},
        columns/count/.style={column name=\textbf{\# of Versions}, column type={r}},
        every head row/.style={after row=\midrule},
        every last row/.style={before row=\midrule},
    ]{plots/https_fail.csv}
    \label{table:https_fail}
\end{table}


==> plots/in_list.tex <==
\begin{table}[h!]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \scriptsize
    \caption{Websites for censorship tests from Citizen Lab.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={category,india},
        columns/india/.style={column name=\textbf{India}, column type={r}},
        columns/category/.style={column name=\textbf{Category}, column type={l}},
        every head row/.style={after row=\midrule},
        %every last row/.style={after row=\bottomrule},
    ]{plots/in_list.csv}
    \label{table:in_list}
\end{table}


==> plots/misc_details.tex <==
\begin{table}[!t]
    \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Search terms in the Miscellaneous category along with the number of unique applications that upload them and the unique domains they are sent to.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns/misc/.style={column name=Search Term, column type={l}},
        columns/packages/.style={column name=Unique Packages, column type={l}},
        columns/hosts/.style={column name=Unique Domains, column type={l}},
        every head row/.style={before row=\hline,after row=\hline},
        every last row/.style={before row=\hline,after row=\hline},
    ]{plots/misc_details.csv}
    \label{table:misc_details}
\end{table}


==> plots/perm_usage_by_sdks.tex <==
\begin{table}[!t]
    \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Access to permission protected API calls by third-party SDKs}
    \resizebox{.5\textwidth}{!}{% <------ Don't forget this %
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns/perm/.style={column name=Perm name, column type={l}},
        columns/app/.style={column name=App only, column type={l}},
        columns/both/.style={column name=App and SDK, column type={l}},
        columns/sdk/.style={column name=SDK Only, column type={l}},
        every head row/.style={before row=\hline,after row=\hline},
        ]{plots/perm_usage.csv} %
        }
        \label{table:perm_usage}
\end{table}


==> plots/pii_hosts.tex <==

\begin{table}[!t]
    \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Entities receiving PII from browsers (* First party).}
    \resizebox{\linewidth}{!}{%
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={host,Ad_id,location_info,device_mac,android_id,total},
        columns/host/.style={column name=\textbf{Destination}, column type={l}},
        columns/location_info/.style={column name=\textbf{Loc}, column type={r}},
        columns/device_mac/.style={column name=\textbf{MAC$\textsubscript{D}$}, column type={r}},
        columns/Ad_id/.style={column name=\textbf{AdID}, column type={r}},
        columns/android_id/.style={column name=\textbf{Android ID}, column type={r}},
        columns/imei/.style={column name=\textbf{IMEI}, column type={r}},
        columns/wifi_name/.style={column name=\textbf{WiFi}, column type={r}},
        % columns/wifi_mac/.style={column name=\textbf{MAC$\textsubscript{W}$}, column type={r}},
        % columns/mitm_cert/.style={column name=Installed Cert, column type={r}},
        columns/device_ip/.style={column name=\textbf{IP}, column type={r}},
        columns/contact_info/.style={column name=\textbf{Contact Info}, column type={r}},
        columns/screen_info/.style={column name=\textbf{Screen Info}, column type={r}},
        columns/total/.style={column name=\textbf{Total}, column type={r}},
        every head row/.style={after row=\midrule},
        every last row/.style={before row=\midrule},
    ]{plots/pii_hosts.csv}}
    \label{table:pii_hosts}
    \ml{Do we need this? It is confusing to have this in the main text and an extended version in the appendix. Also in this case the caption is confusing, we haven o first party? Also, we should have space in the main text.}
    \af{I think we could have the full table here if it its, there's not that
      much of a difference anyways}
\end{table}


==> plots/pii_hosts_extended.tex <==

\begin{table}[!t]
    \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Entities receiving PII from browsers (* First party).}
    \resizebox{\linewidth}{!}{%
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={host,Ad_id,location_info,device_mac,total},
        columns/host/.style={column name=\textbf{Destination}, column type={l}},
        columns/location_info/.style={column name=\textbf{Loc}, column type={r}},
        columns/device_mac/.style={column name=\textbf{MAC$\textsubscript{D}$}, column type={r}},
        columns/Ad_id/.style={column name=\textbf{AdID}, column type={r}},
        columns/android_id/.style={column name=\textbf{Android ID}, column type={r}},
        columns/imei/.style={column name=\textbf{IMEI}, column type={r}},
        columns/wifi_name/.style={column name=\textbf{WiFi}, column type={r}},
        columns/wifi_mac/.style={column name=\textbf{MAC$\textsubscript{W}$}, column type={r}},
        % columns/mitm_cert/.style={column name=Installed Cert, column type={r}},
        columns/device_ip/.style={column name=\textbf{IP}, column type={r}},
        columns/contact_info/.style={column name=\textbf{Contact Info}, column type={r}},
        columns/screen_info/.style={column name=\textbf{Screen Info}, column type={r}},
        columns/total/.style={column name=\textbf{Total}, column type={r}},
        every head row/.style={after row=\midrule},
        every last row/.style={before row=\midrule},
    ]{plots/pii_hosts_extended.csv}}
    \label{table:pii_hosts_extended}
    
\end{table}


==> plots/pii_type.tex <==
\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Various PII categories we look for and the number of unique packages that upload them.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns/category/.style={column name=PII Category, column type={l}},
        columns/apks/.style={column name=\# Browsers, column type={r}},
        columns/packs/.style={column name=\# Packages, column type={r}},
        every head row/.style={after row=\midrule},
        every last row/.style={before row=\midrule},
    ]{plots/pii_type.csv}
    \label{table:pii_type}
\end{table}


==> plots/website_list.tex <==
\begin{table}[!t]
    % \rowcolors{2}{gray!25}{white}
    \centering
    \caption{Websites for censorship tests from Citizen Lab.}
    \pgfplotstabletypeset[
        col sep=comma,
        string type,
        columns={website,category},
        columns/website/.style={column name=\textbf{Website}, column type={l}},
        columns/category/.style={column name=\textbf{Category}, column type={r}},
        every head row/.style={after row=\midrule},
        %every last row/.style={after row=\bottomrule},
    ]{plots/website_list.csv}
    \label{table:website_list}
\end{table}


==> protections.tex <==
\section{Privacy threats and protections}

In this section, we take a deeper look at which browsers are
giving extra protections to their users (\eg blocking
tracking scripts or advertisements) and those that
are generating extra privacy threats for them
(\eg by not handling connection security correctly).

\subsection{Connection Security}

Web browsers are the main point of access to the web for users, and are thus
in charge of correctly implementing security mechanisms such as HTTPS (over TLS).
Failure to do so can compromise user security, and might make them
vulnerable to network attacks.

\para{Certificate validation}
We aim to understand whether browsers that properly validate TLS certificates,
as failing to do so could allow an adversary to create a MITM attack
and observe network traffic. To this end,
we use the methodology presented in
Section~\ref{sec:methodology_dynamic_analysis} but skip installing the
\emph{mitmproxy} root certificate on the mobile device.
Thus, we serve bad certificates to the mobile device when it makes requests
over HTTPS.
With this setup, we instrument the test device to visit a HTTPS website; a
correct implementation of TLS validation would reject the certificate.
Nevertheless, we find that \totalHTTPSFailBrowsers\ (\httpsFailPercentage)
browsers accept this invalid certificate anyway.
These browsers originate from Chinese stores (\totalHTTPSFailAlt) as
well as the Google Play Store (\totalHTTPSFailGPlay, downloaded 
\totalHTTPSFailGPlayDownloads\ times).
These browsers are thus vulnerable to arbitrary TLS interception attacks.
We find that one of these browser displays a warning stating that
there is a possible security problem while loading this test page.
Nevertheless, while the warning is in place, the browser completes loading the
webpage in the background.
Interestingly, \googlePlaySecureBrwosersFail{} of the browsers that are
available on Google Play advertised in their description that they provided
users with ``security-related'' features, yet they fail to validate certificates.


\para{HTTP/S implementation}
We perform a number of tests to understand how browsers implement security
mechanisms such as HTTPS (over TLS), and how they promote connection security.
We first test to see if browsers default to \emph{http} or \emph{https} while
initiating connections, by asking browsers to access a domain without
specifying which protocol to use.
We expect that a browser would always favor \textit{https} in order to better
protect user's privacy. However, we find that only
\domainHttpsBrowsers\ \af{probably better to do percentage here} of the browsers
pick \emph{https} by default.
On the other hand, \domainHttpBrowsers\ of the browsers fail to include
extra protections for the user, as they fetch the website over \emph{http}.

We are also interested in understanding how browsers handle mixed content.
We find that \mixedAllowed\ browsers allow mixed content without notifying the
user in any way, \mixedUpgraded\ browsers upgrade mixed content to be
\emph{https} only and \mixedDisallowed\ browsers block mixed content outright.
\af{Is this correct? It says zero everywhere. if it is correct, then
  we should rewrite accordingly}


\para{Insecure ciphersuites}
Lastly, we analyzed the TLS handshakes browsers in our dataset perform to see
if they support insecure ciphers.
We found that \rc4SupportedBrowsers\ of them support insecure ciphers based on
RC4 ciphers.
We leave a detailed analysis of insecure TLS settings to future work.
\af{I don't see the value of this if we do not go any further,
  I would either remove it or at least include some clearer insights
  on how this can affect users, and how much of a problem
  it can}

\subsection{Content Modification}

Mobile browsers sit between their users and the websites they visit.
We study whether browsers abuse this power to modify content in a way against
users' interests.
To understand such browser modifications, we compare the DOM
displayed for each particular browser with that of the baseline--the actual
website content.
We perform this comparison across various tests, thus measuring browser behavior
for a number of websites, including our honey page as mentioned in
Section~\ref{sec:methodology_dynamic_analysis}. 


\para{Blocking to protect users}
Many mobile browsers advertise themselves as ``secure'' browsers or
``privacy'' browsers. Therefore, it is expected that they take extra
measures to protect user's PII from being accessed by websites.
To measure this, we use the dynamic technique presented in
Section~\ref{sec:methodology_dynamic_analysis} and visit a test page which
contains javascript code to access various types of user data through WebAPIs;
in addition to the previously mentioned website lists. This will
allow us to understand which browsers block such access to sensitive
data and which do not. 

We find that the majority of browsers in our dataset (\trackerBlockers)
\af{better to change to percentage} block tracking scripts.
\af{Any way we can extend here? Do some browsers block more scripts that
  others? What kind of scripts are blocked by all browsers but
  only blocked by a few? Do we have any secure browser that does
  not block tracking scripts?}
\af{Actually after reading everything this seems to be all about
  WebAPIs... Tracking scripts is something very interesting that
  seems to not be included here}

Further, we find that \webViewBrowsers\ browsers use Android \emph{WebViews} to
implement browsing capabilities.
\ml{How did you identify this? So far we are missing any discussion about
  identifying browser engines. Also, this number seems very high. Could it be
  that those browsers use the WebView \emph{in addition} to the browser
  engine, e.g., in libraries for displaying ads or whatnot?}
\af{I might be missing something, but why is this relevant?}
Thus, the WebAPIs they support are limited to those that the API allows them;
they are unable to change browser engine logic, thus forcing them to support a
subset of all WebAPIs.
This inadvertently prevents exposure of various browser information; these
browsers provide access only to the device Accelerometer, Magnetometer and
Battery readings.


We also found \pornBlockers\ browsers blocking links to adult websites, which
are part of our test set. Interestingly, some web browsers are directed at
children and thus have some parental control solutions implemented, which
include the blocking of websites that can be deemed as sensitive for children.

\para{Potentially unwanted modification}
We find a number of browsers that are blocking content unrelated to
PII, something that might be undesired by the user. Namely, we
find that that \amazonBlockers\ browsers block the Amazon referral link we
use in our honeypage. Such links are placed on websites to point
users to an Amazon product, earning a commission when an user purchases
such product. Browsers that block these links are indeed not
helping the user in any way, and are just preventing the webpage
to earn this commission. 

In one case, we found a %\texttt{com.fax.zqdll}%
browser replacing two JavaScript files
(\texttt{jquery.js, getform.js}) with a different version embedded in the
browser itself.
Upon manual analysis, we do not find any indication of this version of the
script containing any tracking capability or privacy invasive behavior.
We also found a browser
% \texttt{com.asus.browser}
injecting a \texttt{inputDetect.js} script from a location within the browser.
When manually verifying the content of this script, it appears to check
whenever a form input is highlighted by the user.
% In another case, we found \texttt{com.vee.project.browser} injecting a 
% \texttt{websocket.js} script from a remote source into a webpage.
% \drc{Seriously, what is this and what did it do? We can't send this without an answer.}
% ~\todo{Did we check whether this does anything}\nv{Maybe see if it has been
% blacklisted by some ad blocker or what VT says about it.}
Last, we found that one browser replaces a Twitter follow
button embedded in one of the visited websites with their custom Twitter widget
code.
When analyzing this custom code, we find that it is indeed a button
that when clicked, composes a tweet that includes custom text related
to the browser itself: \emph{``Sleipnir Mobile for Android |
   https://www.fenrir-inc.com/jp/android/apps/sleipnir-mobile/help/ via
   @fenrir\_official.''}

